Training (Overparametrized) Neural Networks in Near-Linear Time

The slow convergence rate and pathological curvature issues of first-order gradient methods for training deep neural networks, initiated an ongoing effort for developing faster $\mathit{second}$-$\mathit{order}$ optimization algorithms beyond SGD, without compromising the generalization error. Despite their remarkable convergence rate ($\mathit{independent}$ of the training batch size $n$), second-order algorithms incur a daunting slowdown in the $\mathit{cost}$ $\mathit{per}$ $\mathit{iteration}$ (inverting the Hessian matrix of the loss function), which renders them impractical. Very recently, this computational overhead was mitigated by the works of [ZMG19,CGH+19}, yielding an $O(mn^2)$-time second-order algorithm for training two-layer overparametrized neural networks of polynomial width $m$. We show how to speed up the algorithm of [CGH+19], achieving an $\tilde{O}(mn)$-time backpropagation algorithm for training (mildly overparametrized) ReLU networks, which is near-linear in the dimension ($mn$) of the full gradient (Jacobian) matrix. The centerpiece of our algorithm is to reformulate the Gauss-Newton iteration as an $\ell_2$-regression problem, and then use a Fast-JL type dimension reduction to $\mathit{precondition}$ the underlying Gram matrix in time independent of $M$, allowing to find a sufficiently good approximate solution via $\mathit{first}$-$\mathit{order}$ conjugate gradient. Our result provides a proof-of-concept that advanced machinery from randomized linear algebra -- which led to recent breakthroughs in $\mathit{convex}$ $\mathit{optimization}$ (ERM, LPs, Regression) -- can be carried over to the realm of deep learning as well.

==> combine.tex <==
\subsection{Combine}

We use $\| \cdot \|$ to denote the spectral norm of a matrix. We use $\| \cdot \|_F$ to denote the Frobenius of a matrix. We use $\| \|_2$ to denote its entry-wise $\ell_2$ norm.
  
Recall that $G_0 \in \R^{n \times n}$ is Gram matrix at the initialization, we use $G_{0,i,j} \in \R^{b \times b}$ to denote $(i,j)$-th block of $G_0$, $\forall i,j \in [k]$.
Say we have $\wt{G}_{0,i,j} $ satisfies that
\begin{align*}
 (1-\epsilon) G_{0,i,j} \preceq \wt{G}_{0,i,j} \preceq (1+\epsilon)G_{0,i,j}
\end{align*} 
for some sufficiently small $\epsilon \in (0,1)$.

\begin{definition}
We define square matrix $A \in \R^{n \times n}$
\begin{align*}
A = L^{\top}(D - L)^{-1} 
\end{align*}
where $D \in \R^{n \times n}$ is the diagonal block matrix of $G \in \R^{n \times n}$, and $L \in \R^{n \times n}$ is the lower triangular matrix $G \in \R^{n \times n}$ {\small
\begin{align*}
D = 
\begin{bmatrix}
G_{0, 1,1} & 0 & 0 & \cdots & 0 & 0 \\
0 & G_{0, 2,2} & 0 & \cdots & 0 & 0 \\
0 & 0 & G_{0,3,3} & \cdots & 0 & 0 \\
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
0 & 0 & 0 & \cdots & G_{0, k-1, k-1} & 0 \\
0 & 0 & 0 & \cdots & 0 & G_{0, k, k} \\
\end{bmatrix}
L = -
\begin{bmatrix}
0 & 0 & 0 & \cdots & 0 & 0\\
G_{0, 2, 1} & 0 & 0 & \cdots & 0 & 0\\
G_{0, 3, 1} & G_{0,3,2} & 0 & \cdots & 0 & 0\\
\vdots & \vdots &\vdots & \ddots & \vdots & \vdots\\
G_{0, k-1, 1} & G_{0, k-1, 2} & G_{0, k-1, 3} & \cdots &0 &0 \\
G_{0, k, 1} & G_{0, k, 2} & G_{0, k, 2} & \cdots & G_{0,k,k-1} & 0 \\
\end{bmatrix}
\end{align*}}
\end{definition}

\begin{lemma}[Lemma 7 in \cite{cgh+19}]
\label{lem:lemma_7_cgh+19}
Suppose the smallest eigenvalue of the initial Gram matrix $G_0 \in \R^{n \times n}$ satisfies $\lambda_{\min}(G_0) \geq \frac{3}{4}\lambda_0$. Assume $\| J_{W_0, x_l} \|_F = O(1)$ for any $l \in [n]$. Then we have
\begin{align*}
\| A \| \leq 1 - \Omega( \lambda_0^2 / n^2 ) .
\end{align*}
\end{lemma}

\begin{proof}
	\Binghui{TO do}
\end{proof}


%\Binghui{For simplicity, we can think $\mu = 1$, $\delta$ is sufficiently small and $\rho = 1- \lambda^2/n^2$, thus we get $\|\prod_{t=1}^{T}A_t\| \leq (1 - \lambda^2/n^2)^{T}$.}

\begin{lemma}[Lemma 8 in \cite{cgh+19}]\label{lem:lemma_8_cgh+19}
Let $\rho = \| A \|$. Let $A \in \R^{n \times n}$ be diagonalized as $A = P^{-1} Q P$ and $\mu = \| P \|_2 \cdot \| P^{-1} \|_2$. If $\| A_t - A_0 \|_2 \leq \delta$ for $t \leq T$, then
\begin{align*}
\| \prod_{t=1}^T A_t \|_2 \leq \mu \cdot ( \rho + \mu \delta )^T
\end{align*}
\end{lemma}
\begin{proof}
\Zhao{Someone needs to write a proof here.}
\end{proof}

\begin{lemma}[Lemma 9 in \cite{cgh+19}]
\label{lem:lemma_9_cgh+19}
Let $m = \Omega(\frac{\mu^2n^8R^2}{\lambda_0^8})$, for any $(t,i)$-pair, we assume $W_{t',i'} \in B(R)$ for all $i' \in [k]$ when $t' \leq t$ and $i' \in [i]$ when $t' = t$ in the following:

(a) $\min_{ v \in \R^n, \| v \|_2 = 1 } \| ( D - L ) v \|_2 \geq \frac{3}{8} \lambda_0$.

(b) Suppose to $t$, $W_t$ is in $B(R)$, then $\| A_t - A \|_2 \leq ( 1 - \rho(A) ) / ( 2 \mu )$.
\end{lemma}
\begin{proof}
\Zhao{Someone needs to write a proof here.}
\end{proof}


\begin{theorem}[Theorem 2 in~\cite{cgh+19}]\label{thm:cgh19-2}
Let $m$ denote the width of neural network. If 
\begin{align*}
	m = \Omega ( \lambda_0^{-16} \mu^2n^{18} + \lambda_0^{-2} n^2d\log(16n/\delta) ) ,
\end{align*}
Then we have
\begin{align*}
	\| f_{T, k} - y \|_2 \leq \mu \sqrt{n} \cdot ( 1 - \Omega( \lambda_0^2/n^2) )^{T}
\end{align*}
\end{theorem}
\begin{proof}
Notice that we only need to prove that $\|W_{t, i} - W_0\|_F \leq R$, i.e., $W$ does not change too much. %Once this is done, using Lemma~\ref{lem:lemma_8_cgh+19} Lemma~\ref{lem:lemma_7_cgh+19} and , we get

We can upper bound $\| f_t - y \|$ in the following sense:
\begin{align}\label{eq:second1}
	\|f_t - y\| 
	\leq & ~ \|f_0 - y\| \cdot \| \prod_{t-1}^{T} A_t \|  \notag \\
	\lesssim & ~ \sqrt{n} \cdot \| \prod_{t-1}^{T} A_t \| \notag \\
	\leq & ~ \sqrt{n} \cdot \mu ( \rho + \mu \cdot \delta )^{T} &\notag\\
	\leq & ~ \sqrt{n} \cdot \mu ( \rho + \mu \cdot ( 1- \rho) / (2 \mu  ) )^{T}  \notag\\
	= & ~ \sqrt{n} \cdot \mu (  \frac{1}{2}+ \rho / 2 )^T \notag \\
	\leq & ~ \sqrt{n} \cdot \mu  (1 - \Omega( \lambda_0^2 / n^2 ) )^{T}
\end{align}
where the first step follows from triangle inequality, the second step follows from $\|f_0 - y\| = O(\sqrt{n})$, the third step follows from Lemma~\ref{lem:lemma_7_cgh+19} and $\delta = \max_t\{\|A_t - A\|_2\} $, the fourth step follows from $\delta \leq (1 - \rho )/2\mu$ (part b of Lemma~\ref{lem:lemma_9_cgh+19}), and the last step follows from \Zhao{???}.
	
On the other hand, we have
\begin{align*}
R_{t, i} 
= & ~ \|W_{t, i} - W_{t, i+1}\|_{F}\\
= & ~ \|J_{t, i, i}G_{t, i, i, i}^{-1} (f_{t, i, i} - y)\|_2\\
\leq & ~ \frac{\sqrt{n}}{\lambda_0}\|f_{t, i}  - y\|_2  \\ 
\leq & ~ \frac{\sqrt{n}}{\lambda_0}\|U_{t, i}(D_t - L_t)^{-1}\|_2\|f_t - y\|_2\\
\leq & ~ O(\frac{n^{3/2}}{\lambda_0^2})\|f_t - y\|_2\\
\lesssim & ~ \frac{\mu n^2}{\lambda_0^2} (1 -\frac{\lambda_0^2}{n^2})^{T} 
\end{align*}
wwhere the first step follows from ???, the second step follows from ???, the third step follows from $\|J_{t, i, i}\| \approx \sqrt{n}, \|G_{t, i, i, i}^{-1}\|_2\approx 1/\lambda_0$, the forth step follows from ???, the fifth step follows from Eq.~\eqref{eq:second1}.

The second inequality comes from the fact that...
\begin{align*}
\Binghui{to do}
\end{align*}
	
	
	
Taking a summation over $R_{t, i}$, we get
\begin{align*}
	D = \sum_{t=1}^{T}\sum_{i = 1}^{k} R_{t, i} \leq \sum_{t = 1}^{T}k\cdot\frac{\mu n^2}{\lambda_0^2}(1 - \frac{\lambda_0^2}{n^2})^{t} \leq k \cdot \frac{\mu n^4}{\lambda_0^4} \leq \frac{\mu n^5}{\lambda_0^4}.
\end{align*}
where the first step follows from \Zhao{???}, the second step follows from \Zhao{???}, the third step follows from \Zhao{???}, and the last step follows from \Zhao{???}.

Thus, it is sufficient to take $R = \Omega(\mu n^5 / \lambda_0^4) \geq D$. Moreover, by Lemma~\ref{lem:lemma_9_cgh+19}, it suffices to take $m \geq \frac{\mu^2n^8R^2}{\lambda_0^8} = \frac{\mu^2 n^{18}}{\lambda_0^{16}}$. Thus we finish the proof.
\end{proof}
